IC 4665 DANCe I. Members, empirical isochrones, magnitude distributions, present-day system mass function, and spatial distribution

Context. The study of star formation is extremely challenging due to the lack of complete and clean samples of young, nearby clusters, and star forming regions. The recent Gaia DR2 catalogue complemented with the deep, ground based COSMIC DANCe catalogue offers a new database of unprecedented accuracy to revisit the membership of clusters and star forming regions. The 30 Myr open cluster IC 4665 is one of the few well-known clusters of this age and it is an excellent target where to test evolutionary models and study planetary formation. Aims. We aim to provide a comprehensive membership analysis of IC 4665 and to study the following properties: empirical isochrones, distance, magnitude distribution, present-day system mass function, and spatial distribution. Methods. We use the Gaia DR2 catalogue together with the DANCe catalogue to look for members using a probabilistic model of the distribution of the observable quantities in both the cluster and background populations. Results. We obtain a final list of 819 candidate members which cover a 12.4 magnitude range (7 < J < 19.4). We find that 50% are new candidates, and we estimate a conservative contamination rate of 20%. This unique sample of members allows us to obtain a present-day system mass function in the range of 0.02-6 Msun, which reveals a number of details not seen in previous studies. In addition, they favour a spherically symmetric spatial distribution for this young open cluster. Conclusions. Our membership analysis represents a significant increase in the quantity and quality (low-contamination) with respect to previous studies. As such, it offers an excellent opportunity to revisit other fundamental parameters such as the age.

==> Tables/spatial_dist_old.tex <==
\begin{table*}
\centering
\caption{Parameters for the spherically symmetric distributed models. }
    \begin{tabular}{l|ccccccc}
        \hline
		\hline
		Model & $\alpha_c$ & $\delta_c$ & $r_c$ & $\gamma$ & $\alpha$ & $\beta$ & $r_t$ \\ 
		      & [\degr]    & [\degr]    & [pc]  &          &          &         & [pc] \\ 
		\hline
		EFF & $266.574^{+0.071}_{-0.067}$ & $5.438^{+0.087}_{-0.108}$ & $2.38^{+1.32}_{-0.38}$ & $2.133^{+0.324}_{-0.093}$ & -- & -- & -- \\ 
		GDP & $266.579^{+0.053}_{-0.066}$ & $5.438^{+0.107}_{-0.055}$ & $2.19^{+0.56}_{-0.93}$ & $0.18^{+0.34}_{-0.13}$ & $0.20^{+0.60}_{-0.14}$ & $1.81^{+0.16}_{-0.30}$ & -- \\ 
		GKing & $266.586^{+0.051}_{-0.059}$ & $5.433^{+0.103}_{-0.060}$ & $1.95^{+0.48}_{-0.97}$ & -- & $0.22^{+0.61}_{-0.16}$ & $1.67^{+0.19}_{-0.41}$ & $96^{+291}_{-61}$ \\ 
		King & $266.573^{+0.069}_{-0.066}$ & $5.439^{+0.088}_{-0.098}$ & $2.21^{+0.93}_{-0.34}$ & -- & -- & -- & $200^{+650}_{-140}$ \\ 
		OGKing & $266.586^{+0.055}_{-0.071}$ & $5.438^{+0.108}_{-0.070}$ & $1.73^{+0.46}_{-0.57}$ & -- & -- & -- & $51^{+42}_{-12}$ \\ 
		RGDP & $266.582^{+0.053}_{-0.071}$ & $5.434^{+0.112}_{-0.062}$ & $2.04^{+0.46}_{-1.04}$ & -- & $0.22^{+0.55}_{-0.15}$ & $1.82^{+0.18}_{-0.28}$ & -- \\ 
		\hline
		\hline
    \end{tabular}
\label{tab:spatial_distribution}
\end{table*}
